The Proof is in the Pudding: Using Automated Theorem Proving to Generate Cooking Recipes

This paper presents FASTFOOD, a rule-based Natural Language Generation Program for cooking recipes. Recipes are generated by using an Automated Theorem Proving procedure to select the ingredients and instructions, with ingredients corresponding to axioms and instructions to implications. FASTFOOD also contains a temporal optimization module which can rearrange the recipe to make it more time-efficient for the user, e.g. the recipe specifies to chop the vegetables while the rice is boiling. The system is described in detail, using a framework which divides Natural Language Generation into 4 phases: content production, content selection, content organisation and content realisation. A comparison is then made with similar existing systems and techniques.

==> scrap.tex <==
\textbf{Bibliography} \\
Abend, O., Cohen, S. B., and Steedman, M. (2015, June). Lexical Event Ordering with an Edge-Factored  Model. In HLT-NAACL (1161-1171).
 \\
Ahn, Y. Y., Ahnert, S. E., Bagrow, J. P., and Barabási, A. L. (2011). Flavor network and the principles of  food pairing. Scientific reports, 1.
 \\
Aho, S., and Sethi, R. Ullman (1986). Compilers: Principles, Techniques, and Tools. Reading, MA: Addison— XVesley.
 \\
Alama, J., Heskes, T., Kühlwein, D., Tsivtsivadze, E., and Urban, J. (2014). Premise selection for  mathematics by corpus analysis and kernel methods. Journal of Automated Reasoning, 52(2), 191- 213.
 \\
Avigad, J., and Harrison, J. (2014). Formally verified mathematics. Communications of the ACM, 57(4), 66- 75.
 \\
Bateman, J. A. (2002). Natural Language Generation: an introduction and open-ended review of the state of  the art.
 \\
Bayomi, M., Levacher, K., Ghorab, M. R., and Lawless, S. (2015, November). OntoSeg: a novel approach to  text segmentation using ontological similarity. In Data Mining Workshop (ICDMW), 2015 IEEE  International Conference on(1274-1283). IEEE.
 \\
Bledsoe, W. W. (1984). Automated theorem proving: After 25 years (Vol. 89). American Mathematical Soc.. Bridge, J. P., Holden, S. B., and Paulson, L. C. (2014). Machine learning for first-order theorem proving.  Journal of automated reasoning, 53(2), 141-172.
 \\
Bronkhorst, J. (2001). Pānini and Euclid: reflections on Indian geometry. Journal of Indian  Philosophy, 29(1), 43-80.
 \\
Burger [Def 1] (2017). In Cambridge Advanced Learner’s Dictionary and Thesaurus. Retrived August  2017 from http://dictionary.cambridge.org/dictionary/english/burger
 \\
Burger [Def 1, 2] (2017). In Collins English Dictionary. Retrived August 2017
 \\
https://www.collinsdictionary.com/dictionary/english/burger\_1
 \\
Burger [Def 1, 2] (2017). In Meriam Webster Online. Retrieved August 2017 from https://www.merriam webster.com/dictionary/burger
 \\
Burger [Def 1, 2] (2017). In Oxford Living Dictionaries. Retrived August 2017 from  https://en.oxforddictionaries.com/definition/burger
 \\
Buyko E, Tomanek K, Hahn U. Resolution of coordination ellipses in biological named entities using  conditional random fields; Proceedings of the 10th Conference of the Pacific Association for  Computational Linguistics; Melbourne, Australia. September 19–21, 2007; 2007. Pacling. Cardona, G. (1997). Pāṇini: A survey of research. Motilal Banarsidass Publ..
 \\
Carroll, L. (1895). What the tortoise said to Achilles. Mind, 4(14), 278-280.
 \\
Cazzulino, D., Aprea, V. G., Greenwood, J., and Hart, C. (2004). Markup Languages and XML. In Beginning  Visual Web Programming in C\#: From Novice to Professional (271-302). Apress.
 \\
Changhong, G. U. O. (2010). The Application of the Semantic Field Theory in College English Vocabulary  Instruction. Chinese Journal of Applied Linguistics (Foreign Language Teaching and Research  Press), 33(4).
 \\
Chomsky, N. (1956). Three models for the description of language. IRE Transactions on information theory,  2(3), 113-124.
 \\
Chomsky, N. (1957). Syntactic Structures (The Hague/Paris, Mouton) (p. 15). ISBN 3-11-017279-8. Chomsky, N., and Schützenberger, M. P. (1963). The algebraic theory of context-free languages. Studies in  Logic and the Foundations of Mathematics, 35, 118-161.
 \\
CNGL, D. (2014, December). Hierarchical Recursive Tagset for Annotating Cooking Recipes. In 11th  International Conference on Natural Language Processing (p. 353).
 \\
Collins, M. (2003). Head-driven statistical models for natural language parsing. Computational linguistics,  29(4), 589-637.
 \\
Copi, I. M., and Beard, R. W. (Eds.). (2013). Essays on Wittgenstein's Tractatus. Routledge. Cordier, A., Dufour-Lussier, V., Lieber, J., Nauer, E., Badra, F., Cojan, J., Gaillard E., Infante-Blanco L.,  Molli P., Napoli A. and Skaf-Molli, H. (2014). Taaable: a case-based system for personalized  cooking. In Successful Case-based Reasoning Applications-2 (121-162). Springer Berlin  Heidelberg.
 \\
Cruse, D. A. (2002). Hyponymy and its varieties. In The semantics of relationships (3-21). Springer  Netherlands.
 \\
Culleton, T., and Higgs D. (1999). Simply Vegetarian. Dublin: Merlin
 \\
Dale, R. (1988). Generating referring expressions in a domain of objects and processes (Doctoral  dissertation, University of Edinburgh).
 \\
Dale, R. (1989, June). Cooking up referring expressions. In Proceedings of the 27th annual meeting on  Association for Computational Linguistics (68-75). Association for Computational Linguistics. Dale, R. (1992). Generating referring expressions: Constructing descriptions in a domain of objects and  processes. Cambridge, MA: Bradford Books.
 \\
Dale, R., and Haddock, N. (1991). Content determination in the generation of referring expressions.  Computational Intelligence, 7(4), 252-265.
 \\
Denzinger, J., and Schulz, S. (2000). Automatic acquisition of search control knowledge from multiple proof  attempts. Information and Computation, 162(1-2), 59-79.
 \\
Djeraba, C. (2008). Mathematical Tools For Data Mining: Set Theory, Partial Orders, Combinatorics.  Advanced Information and Knowledge Processing. Springer.
 \\
Dufour-Lussier, V., Ber, F. L., Lieber, J., Meilender, T., and Nauer, E. (2012). Semi-automatic annotation  process for procedural texts: An application on cooking recipes. arXiv preprint arXiv:1209.5663. Earley, J. (1970). An efficient context-free parsing algorithm. Communications of the ACM, 13(2), 94-102. Elliott, D., and Keller, F. (2013, October). Image description using visual dependency representations. In  Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing (1292- 1302).
 \\
Evans, G., McDowell, J. H., and McDowell, J. H. (1982). The varieties of reference (100-ff). Oxford:  Clarendon Press.
 \\
Flower, J., Masthoff, J., and Stapleton, G. (2004, March). Generating readable proofs: A heuristic approach to  theorem proving with spider diagrams. In International Conference on Theory and Application of  Diagrams (166-181). Springer Berlin Heidelberg.
 \\
Flynn, S., and Flynn, D. (2016). The World of the Happy Pear. New York, NY: Penguin Random House
 \\
Fontaine, Pascal; Merz, Stephan; Woltzenlogel Paleo, Bruno. Compression of Propositional Resolution  Proofs via Partial Regularization. 23rd International Conference on Automated Deduction, 2011 Fragkou, P. (2017). Applying named entity recognition and co-reference resolution for segmenting English  texts. Progress in Artificial Intelligence, 1-22.
 \\
Frege "On Sense and Reference" ["Über Sinn und Bedeutung"], Zeitschrift für Philosophie und  philosophische Kritik, vol. 100 (1892), pp. 25–50, esp. P
 \\
Frost, R. A., Hafiz, R., and Callaghan, P. C. (2007, June). Modular and efficient top-down parsing for  ambiguous left-recursive grammars. In Proceedings of the 10th International Conference on  Parsing Technologies (109-120). Association for Computational Linguistics.
 \\
Frost, R. A., Hafiz, R., and Callaghan, P. C. (2007, June). Modular and efficient top-down parsing for  ambiguous left-recursive grammars. In Proceedings of the 10th International Conference on  Parsing Technologies (109-120). Association for Computational Linguistics.
 \\
Gaillard, E., Nauer, E., Lefevre, M., and Cordier, A. (2012, August). Extracting generic cooking adaptation  knowledge for the TAAABLE case-based reasoning system. In Cooking with Computers  workshop@ ECAI 2012.
 \\
Galmiche, D. (2000). Connection methods in linear logic and proof nets construction. Theoretical Computer  Science, 232(1), 231-272.
 \\
Galmiche, D., and Marion, J. Y. (1995, May). Semantic proof search methods for ALL-a rst approach. In 4th  Workshop on Theorem Proving with Analytic Tableaux and Related Methods, St Goar am Rhein,  Germany.
 \\
Galmiche, D., and Perrier, G. (1994). Foundations of proof search strategies design in linear logic. Logical  Foundations of Computer Science, 101-113.
 \\
Ganitkevitch, J., Van Durme, B., and Callison-Burch, C. (2013, June). PPDB: The Paraphrase Database. In  HLT-NAACL (758-764).
 \\
Gao, C., and Xu, B. (2013). The application of semantic field theory to English vocabulary learning. Theory  and Practice in Language studies, 3(11), 2030.
 \\
Gavin, P (1987). Italian Vegetarian Cookery. London: Macdonald Optima.
 \\
Geffner, H. (2013). Computational models of planning. Wiley Interdisciplinary Reviews: Cognitive  Science, 4(4), 341-356.
 \\
Georgallides, A. (2015). The unclarity of the notion'object'in the Tractatus (Doctoral dissertation, University  of Sussex).
 \\
Hall, K., and Johnson, M. (2003). Language modeling using efficient best-first bottom-up parsing. In  Automatic Speech Recognition and Understanding, 2003. ASRU'03. 2003 IEEE Workshop on (507- 512). IEEE.
 \\
Hamada, R., Ide, I., Sakai, S., and Tanaka, H. (2000, November). Structural analysis of cooking preparation  steps in Japanese. In Proceedings of the fifth international workshop on on Information retrieval  with Asian languages (157-164). ACM.
 \\
Hamada, R., Miura, K., Ide, I., Satoh, S. I., Sakai, S., and Tanaka, H. (2004, November). Multimedia  integration for cooking video indexing. In Pacific-Rim Conference on Multimedia (657-664).  Berline: Springer.
 \\
Hamada, R., Okabe, J., Ide, I., Satoh, S. I., Sakai, S., and Tanaka, H. (2005, November). Cooking navi:  assistant for daily cooking in kitchen. In Proceedings of the 13th annual ACM international  conference on Multimedia (371-374). ACM.
 \\
Hearst, M. A. (1992, August). Automatic acquisition of hyponyms from large text corpora. In Proceedings  of the 14th conference on Computational linguistics-Volume 2 (539-545). Association for  Computational Linguistics.
 \\
Henshaw, G. (May, 2011). Ginger, lime, edamame, sweet potato burgers. Retrieved July 2017 from  http://www.thefullhelping.com/ginger-lime-edamame-sweet-potato-burgers/
 \\
Hobbs, J.R. and Riloff E (2010). Information extraction. In Handbook of natural language processing (511- 533). Boca Raton: CRC Press.
 \\
Hongxia, X., and Li, Z. (2008, December). An Efficient Extension of Earley's Algorithm for Parsing  Multidimensional Structures. In Computer Science and Software Engineering, 2008 International  Conference on (Vol. 2, pp. 780-783). IEEE.
 \\
Hongxia, X., and Li, Z. (2008, December). An Efficient Extension of Earley's Algorithm for Parsing Multidimensional Structures. In Computer Science and Software Engineering, 2008 International  Conference on (Vol. 2, pp. 780-783). IEEE.
 \\
Jermsurawong, J., and Habash, N. (2015). Predicting the Structure of Cooking Recipes. In EMNLP (781-786). Jette Viethen and Robert Dale [2007] Evaluation in Natural Language Generation: Lessons from Referring  Expression Generation. Traitement Automatique des Langues, 48:1, 141–160.
 \\
Kahn, Arthur B. (1962), "Topological sorting of large networks", Communications of the ACM, 5 (11):  558–562
 \\
Kamp, H., and Reyle, U. (1993). From Discourse to the Lexicon: Introduction to Modeltheoretic Semantics of  Natural Language, Formal Logic and Discourse Representation Theory. Berlin: Kluwer Academic  Publishers.
 \\
Kasami, T. (1965). An efficient recognition and syntax analysis algorithm for context-free languages (No.  Scientific-2). University of Hawaii, Dept of Electrical Engineering
 \\
Kinouchi, O., Diez-Garcia, R. W., Holanda, A. J., Zambianchi, P., and Roque, A. C. (2008). The non equilibrium nature of culinary evolution. New Journal of Physics, 10(7), 073020.
 \\
Koeva, S. (2015). Paraphrasing of Synonyms for a Fine-grained Data Representation. In SEMANTiCS  (Posters and Demos) (79-83).
 \\
Kripke, S., 1977. “Speaker Reference and Semantic Reference,” in French, Uehling, and Wettstein (eds.),  Contemporary Perspectives in the Philosophy of Language, Minneapolis: University of Minnesota  Press,
 \\
Lincoln, P. D., and Shankar, N. (1994, July). Proof search in first-order linear logic and other cut-free sequent  calculi. In Logic in Computer Science, 1994. LICS'94. Proceedings., Symposium on (282-291).  IEEE.
 \\
Lloyd, J. W. (2012). Foundations of logic programming. Springer Science and Business Media. Loos, S., Irving, G., Szegedy, C., and Kaliszyk, C. (2017). Deep Network Guided Proof Search. Proceedings  of 21st International Conference for Logic Programming, Aritificial Intelligence and Reasoning  (85-105).
 \\
Loveland, D. W. (2016). Automated Theorem Proving: a logical basis. Elsevier.
 \\

@misc{henshaw,
  title = {Ginger, lime, edamame, sweet potato burgers},
  howpublished = {\url{http://www.thefullhelping.com/ginger-lime-edamame-sweet-potato-burgers/}},
  note = {Accessed: 2017-08-30}
}
